ARRQP: Anomaly Resilient Real-time QoS Prediction Framework with Graph Convolution

In the realm of modern service-oriented architecture, ensuring Quality of Service (QoS) is of paramount importance. The ability to predict QoS values in advance empowers users to make informed decisions. However, achieving accurate QoS predictions in the presence of various issues and anomalies, including outliers, data sparsity, grey-sheep instances, and cold-start scenarios, remains a challenge. Current state-of-the-art methods often fall short when addressing these issues simultaneously, resulting in performance degradation. In this paper, we introduce a real-time QoS prediction framework (called ARRQP) with a specific emphasis on improving resilience to anomalies in the data. ARRQP utilizes the power of graph convolution techniques to capture intricate relationships and dependencies among users and services, even when the data is limited or sparse. ARRQP integrates both contextual information and collaborative insights, enabling a comprehensive understanding of user-service interactions. By utilizing robust loss functions, ARRQP effectively reduces the impact of outliers during the model training. Additionally, we introduce a sparsity-resilient grey-sheep detection method, which is subsequently treated separately for QoS prediction. Furthermore, we address the cold-start problem by emphasizing contextual features over collaborative features. Experimental results on the benchmark WS-DREAM dataset demonstrate the framework's effectiveness in achieving accurate and timely QoS predictions.

==> 4_3comparisonMethods.tex <==
\subsection{Comparative Techniques}
\begin{table*}[!h]
    \tiny
    \centering
    \caption{Literature survey of State-of-the-art methods (SoA)}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
    \hline
        \multirow{3}{*}{Type}&\multirow{3}{*}{Method} & \multicolumn{8}{c|}{Features} & \multirow{3}{*}{Loss} & \multirow{3}{*}{Summary} \\ \cline{3-10}
        & & \multicolumn{3}{c|}{QoS} & \multicolumn{5}{c|}{Contextual} & &  \\ \cline{3-10}
        & & Data & SM & LF & ID & AS & RG & SP & GL & & \\ \hline\hline
        \multirow{6}{*}{\rotatebox{90}{memory-based}}
        & UPCC \cite{upcc} & \checkmark & \checkmark & - & - & - & - & - & - &  - & QoS prediction based on users similarity \\ \cline{2-12}
        & IPCC \cite{ipcc} & \checkmark & \checkmark & - & - & - & - & - & - & - & QoS prediction based on services similarity \\ \cline{2-12}
        & WSRec \cite{wsrec} & \checkmark & \checkmark & - & - & - & - & - & - & - & Users and services similarity based \\ \cline{2-12}
        & NRCF \cite{nrcf} & \checkmark & \checkmark & - & - & - & - & - & - & - & Proposed a normal recovery based similarity measure  \\\cline{2-12}
        & RECF \cite{recf} & \checkmark & \checkmark & - & - & - & - & - & - & - & Chosen the integrated similarity of users and services  \\\cline{2-12}
        & RACF \cite{racf} & \checkmark & \checkmark & - & - & - & - & - & - & - & Proposed a ratio-based similarity measure \\ \hline
        
        \multirow{15}{*}{\rotatebox{90}{model-based}}
        & NIMF \cite{nimf} & \checkmark & \checkmark & \checkmark & - & - & - & - & - & $L_2$ & Employ Neighborhood Similarity Computation followed by matrix factorization \\\cline{2-12}
        & EMF\_F \cite{emf} & \checkmark & \checkmark & \checkmark & - & - & - & - & - & $L_2$ & A MF framework employ different similarity measurements on the user side and service side to identify neighborhood\\\cline{2-12}
        & MF \cite{llmf} & \checkmark & \checkmark & \checkmark & - & - & \checkmark & - & \checkmark & $L_1$ & Proposed user privacy preserving non-negative matrix factorization framework \\ \cline{2-12}
        & AFM \cite{afm} & \checkmark & \checkmark & - & - & \checkmark & - & \checkmark & - & $L_2$ & Employ factorization machine combined with the attention mechanism on top of Two-Tier Service Filtering\\ \cline{2-12}
        & EFMPred \cite{efm} & \checkmark & - & \checkmark & \checkmark & - & - & - & - & $L_2$ & Introduce embedding technique and employ factorization machine\\ \cline{2-12}
        & CADFM \cite{cadfm} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & - & - & $L_2$ & Leverage FM to capture high-order interactions and MLP for capturing non-linearity \\ \cline{2-12}
        & CSMF \cite{csmf} & \checkmark & - & \checkmark & - & \checkmark & \checkmark & \checkmark & - & $L_2$ & Incorporate contextual information with MF \\ \cline{2-12}
        & Colbar \cite{Colbar} & \checkmark & \checkmark & \checkmark & - & - & - & - & \checkmark & $L_2$ & Proposed MF framework with location-based regularization \\\cline{2-12}
        & DALF \cite{DALF} & \checkmark & - & - & - & - & - & - & - & $L_2$ & Incorporates a density peaks-based clustering method to achieve simultaneous detection of neighborhoods and noises \\  \cline{2-12}
        & TAP \cite{tap} & \checkmark & \checkmark & - & - & - & - & - & - & $L_2$ & Employ K-means clustering for finding trustworthy users/services using a beta reputation system \\   \cline{2-12}
        & CAP \cite{cap} & \checkmark & - & - &  & - & - & - & - & - & Credibility-aware methods to address the unreliable data provided by untrustworthy users using K-Means Clustering \\\cline{2-12}
        & WRAMF \cite{wramf} & \checkmark & - & \checkmark & - & - & - & - & - & $L_2$ & Consider the wide-range impact and employ adaptive learning rate for SGD \\  \cline{2-12}
        & DNM-M \cite{dnmm} & \checkmark & - & - & \checkmark & \checkmark & \checkmark & - & - & $L_1$ & Multi-layer Neural Network for Multiple Attribute QoS prediction with contexts\\  \cline{2-12}
        
        & CMF \cite{cmf} & \checkmark & - & \checkmark & - & - & - & - & - & Cauchy & MF approach taken outliers into consideration \\ \hline


       \multirow{9}{*}{\rotatebox{90}{{\shortstack{memory \\+ \\ model-based}}}}
        & CNR \cite{cnr} & \checkmark & \checkmark & - & - & - & - & - & - & $L_2$ &  Leverage CF with the regression \\ \cline{2-12}
        & DAFR \cite{dafr} & \checkmark & \checkmark & - & \checkmark & - & - & - & \checkmark & $L_2$ & Built denoising auto-encoder, Employ fuzzy clustering, and MLP for QoS prediction \\ \cline{2-12}
        & NCRL \cite{ncrl} & \checkmark & \checkmark & - & \checkmark & \checkmark & \checkmark & - & \checkmark & $L_1$ & Proposed a two-tower deep neural network to learn implicit complex users and services relationships \\ \cline{2-12}
        & CAHPHF \cite{cahphf} & \checkmark & \checkmark & \checkmark & - & - & - & - & \checkmark & $L_2$ & Employ hybrid similarity filtering and hierarchical prediction consisting of CF and MF followed by neural regression  \\ \cline{2-12}
        & TAN \cite{tan} & \checkmark & - & - & \checkmark & \checkmark & - & - & - & $L_2$ & Proposed a topology-aware neural network based on AS \\  \cline{2-12}
        & OffDQ \cite{offdq} & \checkmark & \checkmark & - & - & - & - & - & - & $L_2$ &  Attend High prediction accuracy, Faster prediction time, and High scalability by analyzing various challenges\\ \cline{2-12} 

        & LDCF \cite{ldcf} & \checkmark & - & - & \checkmark & - & \checkmark & \checkmark & - & Huber & Employ MLP and similarity adaptive corrector based on cosine and euclidean similarity between locations \\ \cline{2-12}
        
        & HSA-NET\cite{hsanet} & \checkmark & - & - & - & \checkmark & \checkmark  & \checkmark & \checkmark & $L_2$ & proposed a hidden state aware methods by keeping the users and services privacy  \\ \cline{2-12} 
        
        & TRQP\cite{trqp} & \checkmark & \checkmark & \checkmark & - & \checkmark & \checkmark  & \checkmark & \checkmark & $L_2$ & Identified Grey sheep and proposed Graph-based learning \\ \hline
        \multicolumn{12}{c}{} \\
        \multicolumn{12}{c}{SM - Similarity, LF - Latent users/services features, ID - Users/services identifier, AS - Autonomous systems, RG - Region, SP - Service provider, GL - Geo-location}
    \end{tabular}
    \label{tab:litrature_survey_table}
\end{table*}

==> 4_5analysis_old.tex <==
\subsubsection{Comparison with respect to SoA}
\begin{table*}[!h]
    \centering
    \caption{Comparison of our framework with SoA}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        \hline
        \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{RT-10} & \multicolumn{2}{c|}{RT-20} & \multicolumn{2}{c|}{TP-10} & \multicolumn{2}{c}{TP-20}  \\ \cline{2-9}
         & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE & RMSE \\ \hline \hline
            WSRec \cite{wsrec} & 0.5836 & 1.3298 & 0.4800 & 1.300 &  22.3635& 54.4206 & 19.00 & 48.00 \\\hline
            Colbar \cite{Colbar} & 0.4682 & 1.3300 & 0.4338 & 1.2248 & 15.0145 & 41.3300 & 14.4338 & 40.9786 \\\hline 
            JCM \cite{JCM} &  0.4665 & 1.2505 &  0.4365 & 1.1802 & - & - & - & - \\\hline
            NIMF \cite{nimf} & 0.4554 & 1.2745 & 0.4357& 1.1678 & 16.0542 & 45.9409 & 13.7099 & 41.1689 \\\hline 
            GeoMF \cite{GeoMF} & 0.4610 & 1.1774 & - & - & - & - & - & - \\\hline 
            EFMPred \cite{efm} & 0.4446 & 1.2475 & 0.3900 & 1.1800 & 15.0268 & 44.0291 & 13.00 & 39.00 \\\hline
            CSMF \cite{csmf} & 0.4557 & 1.2315 & 0.4180 & 1.1210 &  26.5850 & 70.0210 & 21.7420 & 61.4380 \\\hline
            LDCF \cite{ldcf} & 0.3670 & 1.233 & 0.3310 & 1.1380 &  12.3820 & 43.4820 & 10.8410 & 38.9980 \\\hline
            DNM-M \cite{dnmm}& 0.3628 & 1.3567 &- &- & 12.9200 & 54.5000 & - & - \\\hline

            JDNMFL \cite{JDNMFL} & 0.3491 & 1.3526 & - & - & 12.6300 & 54.3200 & - & - \\\hline
            
            DAFR \cite{dafr} & 0.3461 & 0.8737 & 0.3404 & 0.8625 & 16.9020 & 41.0620 & 15.5670 & 36.6430 \\\hline
            TAN \cite{tan} & 0.3417 & 1.2917 & - & - & 13.1150 & 54.8793 & - & - \\\hline
            NRCF \cite{nrcf} & 0.3411 & - & 0.2924 & - & - & - & - & - \\\hline 
            NCRL \cite{ncrl} &  0.3385 & 1.2252 & - & - & 11.84 & 41.45 & - & - \\\hline
            HSA\_NET \cite{hsanet} &  0.3270 & 1.1660 &  0.2950 & 1.0910 & - &- & - & - \\ \hline
            MHwA & 0.4013 & 1.4241& 0.3432  & 1.32415 & 15.28485 & 53.9859 & 12.5574 & 47.3566\\ \hline
            SHwoA & 0.3157 & 1.2672 & 0.2578 & 1.1615&  11.2742 & 44.7974 & 9.3988 & 40.2735\\ \hline
            MHwoA  & 0.3143 & 1.2743 & 0.2587 & 1.1383 & 10.7509 & 42.6555 & 8.72855 & 37.8738 \\ \hline
        
    \end{tabular}
    \label{tab:soa1}
\end{table*}

\begin{table*}[!h]
    \centering
    \caption{Comparison of our framework with SoA considering anomaly removal}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
        \multirow{2}{*}{Methods} & Anomaly & \multicolumn{2}{c|}{RT-10} & \multicolumn{2}{c|}{RT-20} & \multicolumn{2}{c|}{TP-10} & \multicolumn{2}{c}{TP-20}  \\ \cline{3-10}
         & removed & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE & RMSE \\ \hline \hline
             MF\cite{llmf} & 10\% & 0.4041 & 0.6120 & 0.4037 &  0.6106 & 16.5509 & 33.8889 & 13.1105 & 27.9648 \\ \hline
             DALF\cite{DALF} & 10\% & 0.3955 & 0.7466 & 0.3439 & 0.6779 & 13.1968 & 27.8531 & 11.9619 & 26.0299 \\\hline
            CAP\cite{cap} & 10\% & 0.3603 & 0.6439 & 0.3521 & 0.6640 & 16.4269 & 32.9558 & 16.3125 & 32.9334 \\\hline
            TAP\cite{tap} & 10\% & 0.3385 & 0.5512 & 0.2843 & 0.4985 & 22.1419 &  43.4987 & 19.8273 & 40.9533 \\\hline
            TRQP \cite{trqp} & 13\% & 0.2540 & - & 0.2520 & - & 10.5760 & - & 9.5660 & - \\\hline
            OffDQ \cite{offdq} & 15\% & 0.2000 & - & 0.1800 & - & 9.1600 & - & 8.6700 & - \\ \hline
            CMF\cite{cmf} & 10\% & 0.1762 & 0.3705 & 0.1524& 0.3599 & 8.4573 & 24.9137 & 7.2501& 20.8927 \\\hline
            MHwA & 10\% & 0.1202 & 0.2917 & 0.10705 & 0.26105 & 5.7032 & 14.57735 & 5.0371 & 14.29785\\ \hline
            SHwoA & 10\% & 0.0963 & 0.3630 & 0.0744 & 0.2691 & 5.0767 & 18.5078 & 4.3573 & 17.4323  \\ \hline
            MHwoA  & 10\% & 0.0930 &0.3556 & 0.0794 & 0.27105 & 4.9652 & 18.3332 & 4.08765 & 16.6755 \\ \hline
    \end{tabular}
    \label{tab:soa2}
\end{table*}

\begin{figure*}
    \centering
    {\includegraphics[width=0.23\linewidth]{fig/diffdensity/rt_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/diffdensity/tp_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/diffdensity/rt_rmse.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/diffdensity/tp_rmse.eps}}
     \caption{Our proposed model results in terms of MAE and RMSE for over four different data densities}
    \label{fig:diffdensity}
\end{figure*}


\subsubsection{Ablation Study}

\begin{figure*}
    \centering
    {\includegraphics[width=0.23\linewidth]{fig/modelAB/rt10_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/modelAB/rt20_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/modelAB/tp10_mae.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/modelAB/tp20_mae.eps}}

    {\includegraphics[width=0.23\linewidth]{fig/modelAB/rt10_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/modelAB/rt20_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/modelAB/tp10_rmse.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/modelAB/tp20_rmse.eps}}
    
    \caption{Model ablation study: The first row and second row represent our model's performance in terms of MAE and RMSE for different models used over four different datasets, respectively.}
    \label{fig:model_ablation}
\end{figure*}


\begin{figure*}
    \centering
    {\includegraphics[width=0.23\linewidth]{fig/featureAB/rt10_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/featureAB/rt20_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/featureAB/tp10_mae.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/featureAB/tp20_mae.eps}}

    {\includegraphics[width=0.23\linewidth]{fig/featureAB/rt10_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/featureAB/rt20_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/featureAB/tp10_rmse.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/featureAB/tp20_rmse.eps}}
    
    \caption{Feature ablation study: The first row and second row represent our model's performance in terms of MAE and RMSE for different features over four different datasets, respectively.}
    \label{fig:feature_ablation}
\end{figure*}



\subsubsection{Gray-sheep Analysis}
\begin{figure*}
    \centering
    {\includegraphics[width=0.23\linewidth]{fig/gs/rt10_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/gs/rt20_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/gs/tp10_mae.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/gs/tp20_mae.eps}}

    {\includegraphics[width=0.23\linewidth]{fig/gs/rt10_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/gs/rt20_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/gs/tp10_rmse.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/gs/tp20_rmse.eps}}
    
    \caption{Grey sheep analysis: By selecting the different values of grey sheep threshold c, we obtain the first row and second row that represent our model's performance in terms of MAE and RMSE over four different datasets, respectively.}
    \label{fig:c_gs}
\end{figure*}

\subsubsection{Cold-start Situation Analysis}

\subsubsection{Outlier Analysis}
\begin{figure*}
    \centering
    {\includegraphics[width=0.23\linewidth]{fig/loss/rt10_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/loss/rt20_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/loss/tp10_mae.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/loss/tp20_mae.eps}}

    {\includegraphics[width=0.23\linewidth]{fig/loss/rt10_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/loss/rt20_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/loss/tp10_rmse.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/loss/tp20_rmse.eps}}
    
    \caption{Impact of different loss function showing the sensitiveness toward outliers}
    \label{fig:loss_function}
\end{figure*}

\subsubsection{Impact of Hyper-parameters}

\begin{figure*}
    \centering
    {\includegraphics[width=0.23\linewidth]{fig/mhgcn/rt10_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/mhgcn/rt20_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/mhgcn/tp10_mae.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/mhgcn/tp20_mae.eps}}

    {\includegraphics[width=0.23\linewidth]{fig/mhgcn/rt10_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/mhgcn/rt20_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/mhgcn/tp10_rmse.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/mhgcn/tp20_rmse.eps}}
    
    \caption{Impact of number of heads in MHGCN}
    \label{fig:hyp_mhgcn}
\end{figure*}

\begin{figure*}
    \centering
    {\includegraphics[width=0.23\linewidth]{fig/mhgat/rt10_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/mhgat/rt20_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/mhgat/tp10_mae.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/mhgat/tp20_mae.eps}}

    {\includegraphics[width=0.23\linewidth]{fig/mhgat/rt10_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/mhgat/rt20_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/mhgat/tp10_rmse.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/mhgat/tp20_rmse.eps}}
    \caption{Impact of number of heads in MHGAT}
    \label{fig:hyp_mhgat}
\end{figure*}

\begin{figure*}
    \centering
    {\includegraphics[width=0.23\linewidth]{fig/gamma/rt10_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/gamma/rt20_mae.eps}}{\includegraphics[width=0.23\linewidth]{fig/gamma/tp10_mae.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/gamma/tp20_mae.eps}}

    {\includegraphics[width=0.23\linewidth]{fig/gamma/rt10_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/gamma/rt20_rmse.eps}}{\includegraphics[width=0.23\linewidth]{fig/gamma/tp10_rmse.eps}}
    {\includegraphics[width=0.23\linewidth]{fig/gamma/tp20_rmse.eps}}
    
    \caption{Impact of $\gamma$ in Cauchy loss}
    \label{fig:gamma}
\end{figure*}

\subsection{Complexity comparison}

